Plain and Simple Inductive Invariant Inference for Distributed Protocols in TLA+

We present a new technique for automatically inferring inductive invariants of parameterized distributed protocols specified in TLA+. Ours is the first such invariant inference technique to work directly on TLA+, an expressive, high level specification language. To achieve this, we present a new algorithm for invariant inference that is based around a core procedure for generating plain, potentially non-inductive lemma invariants that are used as candidate conjuncts of an overall inductive invariant. We couple this with a greedy lemma invariant selection procedure that selects lemmas that eliminate the largest number of counterexamples to induction at each round of our inference procedure. We have implemented our algorithm in a tool, endive, and evaluate it on a diverse set of distributed protocol benchmarks, demonstrating competitive performance and ability to uniquely solve an industrial scale reconfiguration protocol.

==> figures/invgen-algorithm-stavros.tex <==
\algnewcommand{\algorithmicgoto}{\textbf{goto}}%
\algnewcommand{\Goto}[1]{\algorithmicgoto~Line \ref{#1}}%
\begin{algorithmic}[1]
    \State \underline{Inputs}: 
    \State Finite instance of STS $M$; Candidate invariant $Safety$; Lemma invariant repository $\invs$ (typically initially empty).
    \State \underline{Initialization}: 
    \State $Ind \gets Safety$   \label{algolinesafety}
    \State $X \gets GenerateCTIs(M, Ind)$   \label{algolineCTIsinit}
    \State $\invs \gets GenerateLemmaInvariants(M, \invs)$  \label{line:gen-invs}
    % \State Initialize $IsInductive := False$
    % \While{True}
    \State \underline{Main loop:}
    %
    \While{$X \neq \emptyset$}
    \If{$\exists A \in \invs :A$ eliminates at least one CTI in $X$}
		\State pick $A_{max} \in \invs$ that eliminates the most CTIs from $X$ 
		\State $Ind \gets Ind \wedge A_{max}$    \label{algolineIndupdate}
		\State $X \gets X \setminus \{s \in X : s \not\models A_{max}\}$ ;  \label{algolineXupdate}
    \Else \label{algolinecannoteliminate}
		\State either \Goto{line:gen-invs}    \label{algolinegoto}
        \State or \Return ($Ind$, ``Fail: Did not manage to eliminate all CTIs'') ;  \label{invgen-algo:line-fail}
        % \Comment{Return with failure (or go back to Line \ref{line:gen-invs}).}
    \EndIf
    \State $X \gets GenerateCTIs(M, Ind)$    \label{algolineCTIsnew}
    \EndWhile
    \State \Return ($Ind$, ``Success: managed to eliminate all CTIs!'')  \label{algolinesuccess}
\end{algorithmic}


==> figures/invgen-algorithm.tex <==
\algnewcommand{\algorithmicgoto}{\textbf{goto}}%
\algnewcommand{\Goto}[1]{\algorithmicgoto~Line \ref{#1}}%
\begin{algorithmic}[1]
    \State \underline{Inputs}: 
    \State Parameterized system $M$, invariant $Inv$.
    \State \underline{Initialization}: 
    \State $Ind \gets Inv$
    \State $k \gets 0$
    % \State Initialize $IsInductive := False$
    % \While{True}
    \\
    \State $Invs_k \gets GenerateInvariants(M)$ \label{line:gen-invs}
    \State $X_k \gets GenerateCTIs(M, Ind)$
    %
    \If{$X_k = \emptyset$} 
        \State \Return $(\text{True}, Ind)$ 
        % \Comment{Return with invariant candidate.}
    \EndIf 
    \While{$X_k \neq \emptyset$}
    \If{$\exists A \in Invs_k :$ $A$ eliminates some CTIs $C \subseteq X_k$}
    \State Pick $A_{max} \in Invs_k$ that eliminates the most CTIs from $X_k$.
    \Else 
        \State \Return $(\text{False}, Ind)$ or \Goto{line:gen-invs} \label{invgen-algo:line-fail}
        % \Comment{Return with failure (or go back to Line \ref{line:gen-invs}).}
    \EndIf
    \State $Ind \gets Ind \wedge A_{max}$
    \State $X_k \gets X_k \setminus \{c \in X_k : c \nvDash A_{max}\}$ 
    \EndWhile
    % \Comment{Remove counterexamples that violate $A_{max}$}
    % \State Go back to Line \ref{line:gen-invs}.
    \State $k \gets k + 1$
    \State \Goto{line:gen-invs}
    % \EndWhile
\end{algorithmic}

==> related-work-long.tex <==
There are several recently published techniques that attempt to solve the problem of inductive invariant inference for distributed protocols.
% , with varying methodologies and levels of effectiveness. 
The IC3PO tool \cite{goel2021symmetry}, which extended the earlier I4 tool \cite{ma2019i4}, uses a technique based on IC3 \cite{bradley2011sat} with a novel \textit{symmetry boosting} technique that serves to accelerate IC3/PDR and also to infer the quantifier structure of lemma invariants. 
% Similar to our approach, IC3PO also makes use of the small scope hypothesis to avoid undecidability concerns when performing SMT based reasoning. It reasons about finite protocol instances and searches for a protocol cutoff based on a convergence heuristic. 
The fol-ic3 algorithm presented in \cite{koenig2020first} presents another IC3 based algorithm which uses a novel \textit{separators} technique for discovering quantified formulas to separate positive and negative examples during invariant inference. Its scalability, however, was somewhat limited in comparison to other IC3 based tools like IC3PO. SWISS \cite{hance2021finding} is another recent approach that uses an enumerative search for quantified invariants while using the Ivy tool to validate possible inductive candidates. It relies on SMT based reasoning over an unbounded domain, and does not reason directly about finite instances of distributed protocols. DistAI \cite{yao2021distai} uses a similar approach but additionally utilizes a technique of sampling reachable protocol states to filter invariants, which is similar to our approach of executing explicit state model checking as a means to quickly discover invariants. DistAI is limited, however, to learning only universally quantified invariants, and it was not demonstrated that it could solve the larger range of benchmarks achieved by SWISS and IC3PO.  

More broadly, there exist many prior techniques for the automatic generation of program and protocol invariants that rely on data driven or grammar based approaches. Houdini \cite{houdiniflanagan} and Daikon \cite{ernst2007daikon} both use enumerative checking approaches to discover program invariants. FreqHorn \cite{Fedyukovichsyguinvs,FedyukovichAccelerating} tries to discover quantified program invariants about arrays using an enumerative approach that discovers invariants in stages and also makes use of the program syntax. Other techniques \cite{aiken2014cav} have also tried to make invariant discovery more efficient by using improved search strategies based on MCMC sampling \cite{chib1995understanding}.

